Distributed Quantum Computation with Minimum Circuit Execution Time over Quantum Networks

Present quantum computers are constrained by limited qubit capacity and restricted physical connectivity, leading to challenges in large-scale quantum computations. Distributing quantum computations across a network of quantum computers is a promising way to circumvent these challenges and facilitate large quantum computations. However, distributed quantum computations require entanglements (to execute remote gates) which can incur significant generation latency and, thus, lead to decoherence of qubits. In this work, we consider the problem of distributing quantum circuits across a quantum network to minimize the execution time. The problem entails mapping the circuit qubits to network memories, including within each computer since limited connectivity within computers can affect the circuit execution time. We provide two-step solutions for the above problem: In the first step, we allocate qubits to memories to minimize the estimated execution time; for this step, we design an efficient algorithm based on an approximation algorithm for the max-quadratic-assignment problem. In the second step, we determine an efficient execution scheme, including generating required entanglements with minimum latency under the network resource and decoherence constraints; for this step, we develop two algorithms with appropriate performance guarantees under certain settings or assumptions. We consider multiple protocols for executing remote gates, viz., telegates and cat-entanglements. With extensive simulations over NetSquid, a quantum network simulator, we demonstrate the effectiveness of our developed techniques and show that they outperform a scheme based on prior work by up to 95%.

==> 5-step-triangle-1.tex <==
% performing ESs along a path of nodes with minimum expected latency that connect $P_1$ and $P_2$.  } 
We note the following. (i) The edge weights in $G_N$ satisfy the triangular inequality within a constant factor, and thus, the {\em last} step above 
yields a (6/p)-factor approximate solution where $p$ is the probability of success of the swapping operation.\footnote{If $m_i$ and $m_j$ are two memories in the same computer $P$,
then $w'(m_i,m_j)\leq w'(m_i,m_k)+w'(m_k,m_j)$ for any memory $m_k$ in $P$ since 
$w'(m_i,m_j)$ is the time to perform swaps along the shortest path between $m_i$ and $m_j$. If, instead, $m_i$ and $m_j$ 
are in different computers $P_1$ and $P_2$, then, for any $m_k\in P_3$, we 
have~\cite{tqe-22} $w'(m_i,m_j)\leq 3/(2p)(w'(m_i,m_k)+w'(m_k,m_j))$, since
an EP across $P_1$ and $P_2$ can be generated using EPs generated across $(P_2, P_3)$ and $(P_1, P_3)$.}
(ii) The overall algorithm is still a heuristic since the 
conversion from the \minqap to \maxqap does not preserve the approximation factor; however, in our empirical studies, the overall algorithm performed well.

==> Proofs.tex <==
\begin{prf}

Consider a graph $G=(V, E)$ where edges have positive weights and vertices have positive weights as well as a positive cost.
We first define the density of a set of vertices $S\subset V$ as $f(S)=\frac{\sum \limits _{e \in S} w(e)+ \sum \limits _{v \in S} w(v)}{\sum \limits _{v \in S} c(v)}$.
Then, let $S^* \subset V$ be a set of vertices with minimum density.  Note that the subgraph induced by $S^*$ is an optimal solution to the weighted densest subgraph problem with vertex cost. Additionally, let $S(\mathcal{G})$ be the set of vertices in the subgraph returned by $\mathcal{G}$.

We want to show that the algorithm $\mathcal{G}$ is a $2-$approximation algorithm. First, we construct a lower bound on the optimal solution by constructing a feasible solution.

For each edge $ij \in E$ assign the edge to one of $i$ and $j$ arbitrarily. Then, let $\mathcal{W}(v)= \frac{w(v)+\sum \limits_{\text{$e$ assigned to $v$ }} w(e)}{c(v)}$, and let $d_{\text{max}}= \max \mathcal{W}(v)$.   

We first show that $d_{\text{max}}$ is an upper bound on the optimal value. We then show that $d_{\text{max}}$ is upper bounded by twice the value of the solution returned by $\mathcal{G}$.

\para{Claim 1: $d_{\text{max}} \geq f(S^*)$}

\begin{prf}
$f(S^*) \times (\sum \limits _{v \in S^*} c(v)) =\sum \limits _{e \in S^*} w(e)+ \sum \limits _{v \in S^*} w(v) \leq\sum \limits _{v \in S^*} \mathcal{W}(v) c(v) \leq \sum \limits _{v \in S^*} d_{\text{max}}c(v) = d_{\text{max}}  (\sum \limits _{v \in S^*} c(v))$
\end{prf}

While running $\mathcal{G}$, pick the following assignment of edges to vertices: each edge is assigned to the first incident vertex deleted by the algorithm, and $d_{\text{max}}$ is as defined before. 

\para{Claim 2: $d_{\text{max}} \leq 2f(S(\mathcal{G}))$}

\begin{prf}
    Fix an iteration of the greedy algorithm and let $S$ be the current set, with $v_{i_{min}}$ being deleted.  
    \begin{align*}
        \frac{w(v_{i_{min}})+\sum \limits_{\text{$e$ incident on $v_{i_{min}}$ }} w(e)}{c(v_{i_{min}})} &= \min \limits _{v \in S} \frac{w(v)+\sum \limits_{\text{$e$ incident on $v$ }} w(e)}{c(v)}\\
        &\leq \frac{2\sum \limits _{e \in S} w(e)+ \sum \limits _{v \in S} w(v)}{\sum \limits _{v \in S} c(v)}\footnotemark\\
        &\leq 2f(S)
    \end{align*}
    \footnotetext{\text{Given positive numbers $\{a\}_{i \in [n]}$ and $\{b\}_{i \in [n]}$, $\min \limits _{i \in [n]} \frac{a_i}{b_i} \leq \frac{\sum_i a_i }{\sum_i b_i}$. }}
    Note that since $v_{i_{min}}$, all the edges incident on $v_{i_{min}}$ within $S$ are assigned to $v_{i_{min}}$. Therefore, $\mathcal{W}(v_{i_{min}})= \frac{w(v_{i_{min}})+\sum \limits_{\text{$e$ incident on $v_{i_{min}}$ }} w(e)}{c(v_{i_{min}})} \leq 2f(S)$. Since $d_{\text{max}}=\max \limits _{i} \mathcal{W}(v_i)$ over all iterations of $\mathcal{G}$, we have $d_{\text{max}} \leq 2f(S(\mathcal{G}))$.
\end{prf}

From Claim 1 and Claim 2, we have shown that $\mathcal{G}$ is a $2-$approximate algorithm for the weighted densest subgraph problem with vertex cost.
\end{prf}





\begin{prf}
\blue{Proof can be moved to Appendix/removed; should include that there is no wait---circuit execution time.}
Let $E_i$ and $E_j$ be two \EPs such that $E_i \prec_T E_j$. Suppose $E_i \in B_{i'}$ and $E_j \in B_{j'}$  but $B_{j'}$ is generated before $B_{i'}$ in the optimal solution, that is, $j'<i'$. 
Note that $E_i$ becomes available only at the end of batch $B_{i'}$, but has to be consumed before $E_j$. Thus, the \EP $E_j$ has to wait until the whole batch $B_{i'}$ is generated and consumed. As the optimal solution is also a feasible one, we have (i) $latency(B_{j'})+latency(B_{i'})\leq$ $decoherence$ $time$. Additionally, from the submodularity of the latency function, we have (ii) $latency(B_{j'} \cup B_{i'}) \leq$ $latency(B_{j'})+latency(B_{i'})$.  

We now construct a solution $\mathrm{B}$ from $\mathrm{B}^*$ by combining $B_{i'}$ and $B{j'}$ into a single batch. Note that $\mathrm{B}$ is a feasible solution due to inequality (i) \blue{and has a lower aggregate latency }compared to $\mathrm{B}^*$ due to inequality (ii). This is a contradiction. Thus, if $E_i \prec_T E_j$ for any two \EPs $E_i$ and $E_j$, then $E_i$ must be generated in a batch preceding or the same as $E_j$. Each batch $B_i$ must have a contiguous set of \EPs according to the total order.
\end{prf}

==> back-old.tex <==
\section{\bf Background}
\label{sec:back}

\begin{figure}[t]
%\vspace{-0.3in}
\centering
\includegraphics[width=0.35\textwidth]{bg-circuit-eg.pdf}
\caption{Quantum Circuit Representation.}
\vspace{-0.2in}
\label{fig:bg-circuit-eg}
\end{figure}

\para{Qubit States.}
A \emph{qubit} is a \emph{superposition} of classical
states, and is usually written as $\alpha_0\ket{0} + \alpha_1\ket{1}$,
where $\alpha_0$ and $\alpha_1$ are \emph{amplitudes} represented by
complex numbers and such that $\norm{\alpha_0}^2 + \norm{\alpha_1}^2 = 1$.
%%%%%%%%%%%%%%%%%%%%
Here, $\ket{0}$ and $\ket{1}$ are the standard (orthonormal) 
\emph{basis} states; concretely, they
may represent physical properties such as spin (down/up),
polarization, charge direction, etc.
%%%%%%%%
When a qubit such as above is {\em measured}, it collapses to a 
$\ket{0}$ state with a probability of $\norm{\alpha_0}^2$ and to
a $\ket{1}$ state with a probability of $\norm{\alpha_1}^2$.
%%%%%%%%%%%%%%%%%%%%%
In general, a state of an $n$ qubit
system can be represented as $\Sigma_{i=0}^{2^n-1} \alpha_i\ket{i}$
 where ``$i$'' in $\ket{i}$ is $i$'s bit representation. 
\eat{($\Sigma_{i=0}^{2^n-1}\norm{\alpha_i}^2=1$)}

\para{Quantum Circuits.}  Quantum computation is typically abstracted as a 
\emph{circuit}, where horizontal ``wires'' represent \emph{logical qubits} which carry 
quantum data, and operations on the qubits performed by vertical ``gates'' 
connecting the operand wires~\cite{nielsen_chuang_2010} (See Fig.~\ref{fig:bg-circuit-eg}).  Quantum computers (QCs) evaluate a circuit by applying the gates 
in the left-to-right order. 











\softpara{Representation.}  
We represent an \emph{abstract quantum circuit} $C$ over  a set of qubits $\mathcal{Q} = \{q_1, q_2, \ldots\}$ as a sequence of gates $\langle g_1, g_2, \ldots \rangle$ where each $g_t$ is either binary \CNOT gate or a unary gate. (\CNOT gate and unary gates are sufficient to represent any quantum computation). {\em Time instants} are a sequence of numbers associated with the time points in the circuit; see Fig.~\ref{fig:bg-circuit-eg}.
%If $g_k$ is a binary gate, then its represented by $(q_i, q_j)$, the pair of operands for the \textit{CZ} gate, else $g_k$ is represented by $q_i$,  the operand of the unary gate.
%%%%%%%%%%%%%%%%%%%%%%%%%%
We represent binary gates in a circuit as triplets $(q_i, q_j, t)$ where $q_i$ and $q_j$ are the two operands, and $t$ is the time instant of the gate in the circuit, and unary gates as pairs $(q_i, t)$ where $q_i$ is the operand and $t$ is the time instant.


\para{\bf Entanglement Pairs (\EPs).} The state of a 2-qubit system may not always be factorizable into a product of single states. When this is the case, we say that the qubits are \emph{entangled}.  For example, the state $\frac{1}{\sqrt{2}}\ket{00}+\frac{1}{\sqrt{2}}\ket{11}$ is a \emph{maximally entangled state}; qubits entangled in such a state are known as \EPs (entangled pairs). Once entangled, qubits stay entangled even when large distances separate them. 
%%%%%%%%%%%%%%%%%%%%%
\EPs are used for transmitting quantum information via teleportations or executing remote gates as described below. 

\para{Quantum  Network (QN).}
A quantum network is a network of quantum computers (QCs) represented as 
a connected undirected graph with nodes as QCs and edges representing (quantum and classical) direct communication links. 
Each computer $p\in P$ has quantum memory to store qubits; for simplicity, we divide this memory into two parts: {\em data
memory} to store the circuit qubits, and \emph{execution memory} 
to store the qubits (EPs and linked copies) used for communications. 

\subsection{\bf Distribution of Quantum Circuits over QNs}
\label{sec:dqc}

Given a quantum network (QN) and a quantum circuit, our goal is to 
distribute and execute the given circuit over the network with some optimality criteria; in particular, we focus on the optimization objective of the total execution time of the distributed circuit, as it is of most practical significance. Distribution of a circuit
over a network essentially entails two aspects: (i) distributing the
circuit qubits across the QCs/nodes of the QN, and (ii) executing the
``remote'' binary gates (i.e., gates with operands on different QCs) efficiently. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Overhead in the circuit execution time mainly comes from the execution of remote gates, which generally requires a priori \EPs distributed across
the QCs and generation of such EPs entail execution latency. 
%%%%%%%%%%%%%%
Below, we discuss various ways to execute remote gates, and then, in the next subsection, we discuss the generation and distribution of \EPs and their generation latency. 

\para{Executing Remote (Distributed) Quantum Gates.}
To execute such remote gates, we need to bring all operands' values into a single QC via quantum communication. 
%%%%%%%%%%%%%%%%%%%
However, direct/physical transmission of quantum data 
is subject to unrecoverable errors, 
as classical procedures, such as amplified signals 
or re-transmission cannot be applied due to quantum no-cloning~\cite{wooterszurek-nocloning,Dieks-nocloning}.\footnote{Quantum error
correction mechanisms~\cite{muralidharan2016optimal,devitt2013quantum} can be used to mitigate the transmission errors, 
but their implementation is very challenging and is not expected to be used
until later generations of quantum networks.}
%%%%%%%%%%%%%%%%%%%%%%%%%
Fortunately, there are other viable ways to 
communicate qubits across network nodes or execute remote gates, as described below.
%\blue{\emph{No Cloning Theorem}~\cite{wooterszurek-nocloning,Dieks-nocloning} 
%, a %fundamental result in quantum information science, 
%proscribes making \emph{independent} copies of arbitrary qubits. Consequently, it is impossible to recover from communication errors during physical transmission of arbitrary qubits.}
%\eat{This makes robust quantum communication  particularly challenging, especially since classical techniques to achieve robustness, such as amplification and retransmission, rely on copying.  Consequently, the possibility of unrecoverable errors prohibits physical qubit transmission.} 
%\eat{"No cloning" of qubits~\cite{} makes physical transmission of qubits over long distances challenging and even infeasible.}


%We discuss a slight variation of teleportation below---which is what we use in our model.
%\magenta{Cloning prohibits physical} 

%When standard entangled states such as Bell states~\cite{} are available \emph{a priori}, qubit transmission can be done via teleportation, which is accomplished using only classical communication and local gate operations.


\begin{figure*}
  \begin{minipage}[t]{.7\linewidth}
    \includegraphics[width=\linewidth]{figures/Communications.png}%
    \caption{Different quantum communication techniques.}%
    \label{fig:Communication}
  \end{minipage}\hfil
  \begin{minipage}[t]{.3\linewidth}
    \includegraphics[width=\textwidth]{figures/swapping_tree.jpg}
    \caption{Establish \EPs over remote nodes.}
    \label{fig:swapping_tree}
  \end{minipage}%
  \vspace{-0.5cm}
\end{figure*}

\softpara{Teleportation.}
An alternative approach to physically transmit a qubit from a node
$A$ to $B$ is via \emph{teleportation}~\cite{Bennett+:93} 
which requires an a priori distribution of an \EP over $A$ and $B$. 
See Fig.~\ref{fig:Communication}(a).
With an \EP distributed over $A$ and $B$, teleportation of a qubit 
state from $A$ to $B$ can be accomplished using classical 
communication and local gate operations while consuming/destroying 
the \EP. 
Teleportation can be used to bring operands of a remote gate
to a single QC for local execution. 

\softpara{Telegates.} 
One way to execute remote gates without communicating the
gate operands are via the telegate protocol~\cite{Caleffi}. 
The telegate protocol (see Fig.~\ref{fig:Communication}(b))
is a sequence of local operations that effectuates the execution of
a remote \CNOT gate with operands at nodes $A$ and $B$; the protocol
requires an a priori distribution of an \EP over $A$ and $B$.

\softpara{Cat-Entanglement: Creating ``Linked Copies'' of a Qubit.}
Yet another approach to execute remote gates is by creating \emph{linked read-only copies} of a qubit across QCs via \emph{cat-entanglement} operations~\cite{Eisert+:00,YimsiriwattanaL:05}. Creating a linked copy of a qubit $q$ at node $A$ to a node $B$
requires a priori distribution of an \EP over $A$ and $B$.
See Fig.~\ref{fig:Communication}(c).
The linked copy at $B$ can be used to execute binary gates 
where $q$ is the (read-only) control qubit, 
until a unary operation needs to be executed on $q$. 
When a unary operation needs to be executed on $q$, a disentanglement
operation is done, which destroys the linked copies, and then, the unary
operation can be done on the original qubit $q$ at $A$.
%%%%%%%%%%%%%%%%%%%%%%%%

\softpara{Teleportation vs.\ Telegates vs.\ Cat-Entanglements.}
First, observe that each of these three communication protocols requires a single
EP. Teleportation transports the qubit operand to the computer where the
gate is executed. In contrast, the telegate protocol executes a remote gate
without moving qubits. The main advantage of cat-entanglement is that one cat-entanglement (and, thus, one linked copy) can sometimes be used to execute
several binary gates; however, we need a non-trivial algorithm to determine
the optimal or near-optimal set of cat-entanglements to execute the given set
of remote gates. Moreover, cat-entanglements are best 
used for circuits with only \cz binary gates (see \S\ref{sec:ce}).
%%%%%%%%%%%%%%%%%%%%%%%
This paper considers both telegates and cat-entanglements (\S\ref{sec:ce}) 
for executing remote gates. The use of teleportations leads to dynamic qubit 
allocation (see \S\ref{sec:problem}), which requires more a sophisticated problem 
formulation
and solution, and is thus deferred to our future work.

\subsection{\bf Generating \EPs over Remote Nodes}
\label{sec:eps}

% \begin{figure}[t]
% \vspace{-0.3in}
% \centering
% \includegraphics[width=0.35\textwidth]{figures/Swapping Tree.png}
% \caption{Establishing \EPs over remote nodes.}
% \vspace{-0.2in}
% \label{fig:swapping_tree}
% \end{figure}

\red{Can be shortened.}
One simple way to have an \EP distributed over remote nodes $A$ and $B$ is to generate an \EP locally (at some node) and transport both the qubits to $A$ and $B$ respectively; however, this involves direct communication of qubits which may not
be feasible due to irrecoverable errors over large distances.
%%%%%
To circumvent the above challenge, to distribute an \EP over remote nodes $A$ and $B$, we generate \EPs over larger and larger distances from shorter-distance \EPs using a sequence of ``entanglement-swapping'' operations. 
%%%%%%%%%%%%%%%
An entanglement swapping (\es) operation can be looked up as being performed over a triplet of nodes $(A, B, C)$ 
with two \EPs available at the 
two pairs of nodes $(A, B)$ and $(B,C)$; it results in an \EP over the pair
of nodes $(A, C)$, by essentially teleporting the first qubit in $B$ (the one entangled with $A$) to $C$ using the 2nd \EP over $(B,C)$.
%%%%%%%%%%%%%%%%%%%%%%%

In general, an \EP over a pair of remote nodes $A$ and $B$ can be generated by
a sequence of \es operations over the \EPs over adjacent-nodes along a path
from $A$ to $B$.
%%%%%%
For example, consider a path of nodes $x_0, x_1, x_2, x_3, x_4, x_5$, with an \EP
between every pair of adjacent nodes $(x_i, x_{i+1})$. Thus, each node $x_i$
($1 \leq i \leq 4$) has two qubits, one of which is entangled with $x_{i-1}$ 
and the other with
$x_{i+1}$. Nodes $x_0$ and $x_5$ have only one qubit each.
%%%%%%%%%%%%%%%%%
To establish an \EP 
between $x_0$ and $x_5$, we can perform a sequence of entanglement
swappings (\ess) over the following triplet of nodes (see Fig.~\ref{fig:swapping_tree}):
(i) \es over  $(x_1, x_2, x_3)$ to yield an \EP over $(x_1, x_3)$,
(ii) \es over  $(x_1, x_3, x_4)$ to yield an \EP over $(x_1, x_4)$,
(iii) \es over  $(x_1, x_4, x_5)$ to yield an \EP over $(x_1, x_5)$,
(iv) \es over  $(x_0, x_1, x_5)$ to yield an \EP over $(x_0, x_5)$.
%%%%%%%%%%%%%%%%%%%%%
Similarly, the sequence of \es over the following triplets would also 
work: $(x_2, x_3, x_4)$, $(x_2, x_4, x_5)$, $(x_0, x_1, x_2)$, 
$(x_0, x_2, x_5)$. 
%%%%%%%%%%%%%%%%%%%%%
In general, given a path $P = s \leadsto d$ from $s$ to $d$, 
any complete binary tree (called a \textit{swapping tree}) over 
the ordered links in $P$ gives a way to generate an \EP over $(s, d)$.
%%%%%%%%%%%%
Different swapping trees over the same path $P$ can incur different generation
latencies.

\softpara{Generation Latency of an \EP or \EPs.}
The stochastic nature of \es operations
means that an \EP at the swapping tree's root will be successfully 
generated only after many failed attempts and hence accumulates significant latency.
We refer to this latency as the \textit{generation latency} of the \EP 
(using the given tree). 
%%%%%%%%%%%%%%%%%%%%%%%%
To generate a set $S$ of \EPs concurrently, we need to allocate the network 
resources appropriately for generating each \EP in the set $S$. In general,
the total latency incurred in generating a set $S$ of \EPs is at most the sum
of the latencies of generating them independently (as they can always be 
generated
one at a time).



% * Reality.
% * How are we handling it? Decoherence Threshold. Fidelity -- Purifications.
% * How do we write it?
%     . Start with TQE para.
%         . Reality. Introduce purification.
%         . We handle the two issues in the following ways?

\subsection{\bf Decoherence and Fidelity}

\emph{Fidelity} is a measure of how close a realized state is to the ideal. The fidelity of a quantum state decreases over time due to interaction with the environment and gate operations. Time-driven fidelity degradation is called \emph{decoherence}. To bound decoherence, we limit the aggregate time a qubit spends in a quantum memory before being consumed by the {\em decoherence threshold} of $\tau$ seconds.
%%%%%%%%%%%%%%%%%%%%%%
% To combat fidelity degradation, one can use entanglement purification \cite{purification} and error correction \cite{error} techniques. 
% In our work, 
We address fidelity degradation by using entanglement purification~\cite{Briegel1998QuantumRT} techniques which entails using multiple copies of an EPs to improve its fidelity.


% Daei et al.~\cite{Daei2020OptimizedQC} consider the problem of reducing teleportation cost in distributed quantum circuits. The main idea behind their paper is to
% construct an appropriate graph over qubits and use the Kernighan-Lin graph bisection algorithm iteratively to partition the graph into $k$ parts. Then, each part is assigned to a different quantum computer, and every non-local gate is
% executed using teleportations. In another work, Moghadam et al.~\cite{zomorodi2018optimizing} consider the special case of only two computers with the qubits assignment across the computers
% is already given; for this special case, they provide an exponential time algorithm that finds the minimum number of teleportations to execute all binary gates. Finally, Nikahd et al.~\cite{Nikahd_2021} first segregate the binary gates into ``levels,'' then determine the best partition of qubits for each level by solving an integer linear program. 

% \blue{Some works have addressed the DQC problem using cat-entanglements as the only means of communication. For example,~\cite{andres2019automated} poses} the \dqc problem as a balanced hypergraph partitioning problem and gives a heuristic based on hypergraph min-cut. For a simplified setting,~\cite{g2021efficient} presents a two-step algorithm for the \dqc problem, wherein
% the first step determines the partitioning of qubits to computers through balanced graph partitioning and the second step minimizes the number of cat-entanglement operations via
% an iterative greedy approach. 
% %%%%%%%%%%%%%%%%%%%%%
% Finally, in ~\cite{dqc-gen}, the authors allow use of {\em both} 
% teleportations and cat-entanglements to communicate quantum states, and
% consider the general \dqc problem with both storage and execution memory constraints on computers. 


%%%%%%%%%%%%%


% \begin{itemize}
%     \item A change in the home-computer function at time instant $t$.
%     \item Occurs only before binary gates.
%     \item Going from one partition to the other, what is a way to find the minimum number of teleportations from partition 1 to partition 2?
%     \item Assuming all computers have a gap of at least 1, will the above                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                               
% \end{itemize}
